Complementarity of Bs->mu+mu- and B-> K l+l- in New Physics searches

This year, LHC provided a very stringent bound on Br(Bs->mu+mu-), bringing it closer to the value predicted by the Standard Model (SM). Bs->mu+mu- was believed to be the golden mode at LHCb to find SUSY because a large enhancement was expected in the regime of moderate and large values of tanb. Other scenarios are still possible and a correlation with other decay channels is needed. We show that a complementary information on New Physics (NP) can be obtained model-indepedently from the B-> K l+l- decay mode. We provide a prediction Br(B-> K l+l-) based on the first lattice QCD results for all three relevant form factors, f0(q^2), f+(q^2) and fT(q^2). We were then able to provide the model-independent bounds on the complex couplings to scalar and pseudoscalr operators in the b->s sector.

==> bib_sample.tex <==
%%%%%%%%%%%%%%%
\begin{thebibliography}{999}
\vspace*{-0.25cm}
%%%%%%%%%%%%%%%%%%%
% QSSR SVZ & REVIEW
%%%%%%%%%%%%%%%%%%%
\bibitem{SVZ} M.A. Shifman, A.I. and Vainshtein and V.I. Zakharov,
Nucl. Phys. {\bf B147} (1979) 385 .
\bibitem{SNB} For a review and references to original works, see
e.g., S. 
Narison, {\it QCD as a theory of hadrons,
Cambridge Monogr. Part. Phys. Nucl. Phys. Cosmol.} {\bf 17} 
(2002) 1-778
[hep-h/0205006]. 

%%%%%%%%%%%%%%%%%%%
% EXPERIMENT
%%%%%%%%%%%%%%%%%%%
\bibitem{PDG} For a review, see e.g. PDG 08, C. Amsler et al., {\it Phys. Lett.} {\bf B 667} (2008) 1.
\bibitem{BELLE}  S.-K. Choi  {\it et al.} [Belle Collaboration],   
Phys. Rev. Lett. {\bf 91}, 262001 (2003).


\end{thebibliography}
\end{document}

